$k$-Convex Polyominoes by Semi-perimeter

We give the conjectured solution for the generating function of $k$-convex polyominoes, enumerated by semi-perimeter. The solution was obtained from the analysis of enumeration data that we generated.

==> eptcsdata.tex <==
\providecommand{\firstpage}{66}
%\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2026\\
%EPTCS ??, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
%doi:\href{https://dx.doi.org/10.4204/EPTCS.??.10}{10.4204/EPTCS.??.10}}
\pdfoutput=1
%\providecommand{\firstpage}{}
%\providecommand{\publicationstatus}{},
%doi:\href{https://dx.doi.org/10.4204/EPTCS.??.10}{10.4204/EPTCS.??.10}}
%\pdfoutput=1
